Runtime vs Scheduler: Analyzing Dask's Overheads

Dask is a distributed task framework which is commonly used by data scientists to parallelize Python code on computing clusters with little programming effort. It uses a sophisticated work-stealing scheduler which has been hand-tuned to execute task graphs as efficiently as possible. But is scheduler optimization a worthwhile effort for Dask? Our paper shows on many real world task graphs that even a completely random scheduler is surprisingly competitive with its built-in scheduler and that the main bottleneck of Dask lies in its runtime overhead. We develop a drop-in replacement for the Dask central server written in Rust which is backwards compatible with existing Dask programs. Thanks to its efficient runtime, our server implementation is able to scale up to larger clusters than Dask and consistently outperforms it on a variety of task graphs, despite the fact that it uses a simpler scheduling algorithm.

==> task-scheduling.tex <==
In this text, we assume that a computation is given as a task graph -- an acyclic graph of tasks, where arcs represents dependencies. A task needs all dependencies to be finished before it can be executed.
Tasks are processed by working nodes that do not share memory, hence when a task is scheduled on a worker,
all results of a dependencies have to be transferred to this worker.

We are focused on centralized scheduling, i.e. there is a server process that distributes task to workers. Workers may communicate directly for data transfers; however, assignments of task and notification of their completion is always communicated through the server.

For the purpose of this we separate server process into two parts: scheduling algorithm and \emph{runtime} -- an actual implementation of the server (efficient handing connections, communication of scheduler decision to workers, receives notification of finished tasks, etc).

Finding the optimal schedule for a task graph is NP-hard even for very restricted formulations (even without transfer costs)~\cite{Ullman1975}. Plenty of heuristics have been proposed to tackle this problem, ranging from list-based scheduling to genetic algorithms. Many surveys and comparisons of scheduling algorithms were published in~\cite{hlfet1974,kwok1998benchmarking,hagras2003static,wang2018list}.

Main \emph{contribution} of this text: We show that a fast runtime is more important that a clever scheduler. We demonstrate this on fact on \\dask{} case study.
Moreover, we show that in many situations, a random scheduler with a fast runtime surpasses
orginal \\dask{} runtime and scheduler.
We argue that for efficient distributed system with a central scheduler, the efficiency of the runtime must be handled with the same care as the scheduling algorithm itself.
\todo[inline]{Contribution ze jsme zmereli rezii dasku skze zero worker?}

First, we show that a fully random scheduler provides comparable make span in many cases. It indicates that in our use case, an actual schedule has lesser impact than we expected. It also shows that random scheduling can be used as reasonable baseline when we want to compare efficiency of server implementation.

For our experiments we use \dask{} 2.8.1 with small modifications described in section \ref{sec:evaluation}.
We have also reimplemented part of \\dask{} server
from scratch in Rust to evaluate overhead caused by current Python implementation of server. \rsds{} implements only a subset of functionality of the original \dask{} server; however, it contains all core functionality and it is able to execute all benchmarks presented in this text. We are also not aware of any missing functionality which implementation would have a large performance impact.

We have also implemented trivial \dask{} worker in Rust that do not perform any actual computation but communicates like a real worker. We call it \emph{zero worker}.
It is used to measure scheduler and communication overhead in an ideal environment with almost infinitely fast workers and data transfers. For distinction, we use term ``standard worker'' for original Python \dask{} worker. 

In experiments we are using standard worker except when the zero worker is explicitly mentioned.
We are focused on performance of server component. We did not 
do any performance changes of client or worker code and they are used as it is.
The only changes was a simplification of the communication protocol (Section~\todo{ref}), but this change has no performance implication.
